Negotiation Games (with abstract)

Negotiations, a model of concurrency with multi party negotiation as primitive, have been recently introduced in arXiv:1307.2145, arXiv:1403.4958. We initiate the study of games for this model. We study coalition problems: can a given coalition of agents force that a negotiation terminates (resp. block the negotiation so that it goes on forever)?; can the coalition force a given outcome of the negotiation? We show that for arbitrary negotiations the problems are EXPTIME-complete. Then we show that for sound and deterministic or even weakly deterministic negotiations the problems can be solved in PTIME. Notice that the input of the problems is a negotiation, which can be exponentially more compact than its state space.

==> tikz/FDM_PingPong.tex <==
\tikz{
\nego[text=FDM,id=n0,spacing=2]{0,0}
\node[left = 0cm of n0_P0, font=\large] {$n_0$};
\nego[text=FD,id=n1]{0,-2}
\node[right = 0cm of n1_P1, font=\large] {$n_{\text{\scriptsize{FD}}}$};
\nego[text=DM,id=n2]{3,-3.5}
\node[above = 0cm of n2_P0, font=\large] {$n_{\text{\scriptsize{DM}}}$};
\nego[text=D,id=nd]{2,-4.5}
\node[above left = -0.2cm and 0cm of nd_P0, font=\large] {$n_\text{\scriptsize{D}}$};
\nego[text=FDM,id=nf,spacing=2]{0,-6.5}
\node[left = 0cm of nf_P0, font=\large] {$n_f$};
\pgfsetarrowsend{latex}
\draw (n0_P0) -- (n1_P0);
\labelEdge[start=n0_P0,end=n1_P0,dist=0.7,shift={-0.3,0}]{st}
\draw (n0_P1) -- (n1_P1);
\labelEdge[start=n0_P1,end=n1_P1,dist=0.7,shift={-0.4,0}]{st}
\draw (n0_P2) -- (n2_P1);
%\draw (4,-1) to [out=-10,in=10] (nf_P2);
\draw (4,-1) arc (70:-65:2.92cm);
%\draw (4,-1) to [bend left=90] (nf_P2);
\labelEdge[start=n0_P2,end=n2_P1,dist=0.7,shift={0.3,0}]{st}
\draw (n1_P0) -- (nf_P0);
\labelEdge[start=n1_P0,end=nf_P0,dist=1.5,shift={-0.3,0}]{y,n}
\draw[-] (n1_P0) -- (-1,-2.5);
%\draw (-1,-2) to [bend left=90] (n1_P0);
\draw (-1,-2.5) arc(225:32:0.6cm);
\draw (-1,-2.5) -- (nf_P0);
\labelEdge[start=n1_P0,end={-1,-2.5},dist=0.5,xy=x,shift={-0.15,0.15}]{am}
\draw (n1_P1) -- (n2_P0);
\labelEdge[start=n1_P1,end=n2_P0,xy=x,dist=1.1,shift={0.1,0.2}]{am}
\draw (n1_P1) -- (1,-5.3) -- (nf_P1);
\labelEdge[start=n1_P1,end={1,-4.3},dist=2.8,shift={0.3,0}]{y,n}
\draw (n2_P0) -- (nd_P0);
\labelEdge[start=n2_P0,end=nd_P0,dist=0.3,shift={-0.3,0}]{af}
\draw (n2_P0) -- (3,-5.3) -- (nf_P1);
\labelEdge[start=n2_P0,end={3,-4.3},dist=1.3,shift={-0.3,0}]{y,n}
\draw (n2_P1) -- (nf_P2);
\labelEdge[start=n2_P1,end=nf_P2,dist=1,shift={0.3,0}]{y,n}
\draw[-] (n2_P1) -- (5,-4);
\draw (5,-4) arc(-45:147:0.6cm);
\draw (5,-4) -- (nf_P2);
\labelEdge[start=n2_P1,end={5,-4},dist=0.5,xy=x,shift={0.15,0.15}]{af}
\draw (nd_P0) -- (n1_P1);
\labelEdge[start=nd_P0,end=n1_P1,dist=1,shift={0.2,0}]{c}
\draw (nd_P0) -- (nf_P1);
\labelEdge[start=nd_P0,end=nf_P1,dist=1,shift={0.3,0}]{gu}
}

==> tikz/FDM_acyclic_released.tex <==
\tikz{
\nego[text=FDM,id=n0,spacing=2]{0,0}
\node[left = 0cm of n0_P0, font=\large] {$n_0$};
\nego[text=FD,id=n1]{0,-2}
\node[left = 0cm of n1_P0, font=\large] {$n_1$};
\nego[text=DM,id=n2]{3,-4}
\node[left = 0cm of n2_P0, font=\large] {$n_2$};
\nego[text=M,id=n3]{4,-2}
\node[left = 0.2cm of n3_P0, font=\large] {$n_3$};
\nego[text=FDM,id=nf,spacing=2]{0,-6}
\node[left = 0cm of nf_P0, font=\large] {$n_f$};
\pgfsetarrowsend{latex}
\draw (n0_P0) -- (n1_P0);
\labelEdge[start=n0_P0,end=n1_P0,dist=0.7,shift={-0.3,0}]{st}
\draw (n0_P1) -- (n1_P1);
\labelEdge[start=n0_P1,end=n1_P1,dist=0.7,shift={-0.4,0}]{st}
\draw (n0_P2) -- (n3_P0);
\labelEdge[start=n0_P2,end=n3_P0,dist=0.7,shift={-0.3,0}]{st}
\draw (n3_P0) -- (n2_P1);
\labelEdge[start=n3_P0,end=n2_P1,dist=0.7,shift={-0.3,0}]{$r_1$}
\draw (n3_P0) -- (4.5,-2.5) -- (4.5,-5.5) -- (nf_P2);
\labelEdge[start=n3_P0,end=n2_P1,dist=0.7,shift={0.8,0}]{$r_2$}
\draw (n1_P0) -- (nf_P0);
\labelEdge[start=n1_P0,end=nf_P0,dist=1.5,shift={-0.6,0}]{y,n,am}
\draw (n1_P1) -- (n2_P0);
\labelEdge[start=n1_P1,end=n2_P0,dist=0.5,shift={0.5,0}]{am}
\draw (n1_P1) -- (nf_P1);
\labelEdge[start=n1_P1,end=nf_P1,dist=1.3,shift={0.3,0}]{y,n}
\draw (n2_P0) -- (nf_P1);
\labelEdge[start=n2_P0,end=nf_P1,dist=0.5,shift={-0.3,0}]{y,n}
\draw (n2_P1) -- (nf_P2);
\labelEdge[start=n2_P1,end=nf_P2,dist=0.5,shift={-0.35,0}]{y,n}
}


==> tikz/TM_reductionUnsoundInit.tex <==
\tikz{
%atoms
\nego[id=n0,ports=3]{0,0}
\port[text=h]{n0_P0}
\node[left = 0cm of n0_P0, font=\large] {$n_0$};
\nego[id=n0e0,ports=2]{0,-2}
\port[text=h]{n0e0_P0}
\node[left = 0cm of n0e0_P0, font=\large] {$n_{0,\square}$};
\nego[id=n0a0,ports=2]{2,-2}
\port[text=h]{n0a0_P0}
\node[right = 0cm of n0a0_P1, font=\large] {$n_{0,a}$};
\nego[id=n0e1,ports=2]{0,-3}
\port[text=h]{n0e1_P0}
\node[left = 0cm of n0e1_P0, font=\large] {$n_{1,\square}$};
\nego[id=n0a1,ports=2]{2,-3}
\port[text=h]{n0a1_P0}
\node[right = 0cm of n0a1_P1, font=\large] {$n_{1,a}$};
\nego[id=n0er,ports=2]{0,-4}
\port[text=h]{n0er_P0}
\node[left = 0cm of n0er_P0, font=\large] {$n_{reject,\square}$};
\nego[id=n0ea,ports=2]{0,-5}
\port[text=h]{n0ea_P0}
\node[left = 0cm of n0ea_P0, font=\large] {$n_{accept,\square}$};
\nego[id=n1e1,ports=2]{6,-3}
\port[text=h]{n1e1_P0}
\node[left = 0cm of n1e1_P0, font=\large] {$n_{1,\square}$};
\nego[id=n1a1,ports=2]{8,-3}
\port[text=h]{n1a1_P0}
\node[right = 0cm of n1a1_P1, font=\large] {$n_{1,a}$};
\nego[id=n1er,ports=2]{6,-4}
\port[text=h]{n1er_P0}
\node[left = 0cm of n1er_P0, font=\large] {$n_{reject,\square}$};
\nego[id=n1ar,ports=2]{8,-4}
\port[text=h]{n1ar_P0}
\node[right = 0cm of n1ar_P1, font=\large] {$n_{reject,a}$};
\nego[id=nf,ports=3]{0,-7}
\port[text=h]{nf_P0}
\node[left = 0cm of nf_P0, font=\large] {$n_f$};
%edges
\pgfsetarrowsend{latex}
%initial edges
\draw (n0_P0) -- (n0e0_P0);
\draw (0,-1) -- (n0a0_P0);
\draw (n0_P1) -- (n0e0_P1);
\draw (1,-1) -- (1.5,-1.5) -- (1.5,-2) -- (1.5,-3) -- (n0e1_P1);
\draw (1.5,-3) -- (1.5,-4) -- (n0er_P1);
\draw (1.5,-4) -- (1.5,-5) -- (n0ea_P1);
\draw (n0_P2) -- (7,0) -- (n1e1_P1);
\draw (7,-2) -- (7.5,-2.5) -- (7.5,-4) -- (n1er_P1);
%acceptance edges
\draw (n0ea_P0) -- (nf_P0);
\draw (n0ea_P1) -- (nf_P1);
\draw[dashed] (6,-5) -- (nf_P2);
}

==> tikzMacros.tex <==

\usepackage{tikz}
\usetikzlibrary{calc,arrows,automata,positioning,fit}
\usepackage{xstring}
\usepackage{keyval}
\usepackage{xifthen}

\makeatletter
%Extract x and y from coordinate
\newcommand{\getxy}[3]{%
  \tikz@scan@one@point\pgfutil@firstofone#1\relax
  \edef#2{\the\pgf@x}%
  \edef#3{\the\pgf@y}%
}
% LABELEDGE
% ========= KEY DEFINITIONS =========
\define@key{labelEdge}{start}{\def\labelEdge@start{#1}}
\define@key{labelEdge}{end}{\def\labelEdge@end{#1}}
\define@key{labelEdge}{dist}{\def\labelEdge@dist{#1}}
\define@key{labelEdge}{xy}{\def\labelEdge@xy{#1}}
\define@key{labelEdge}{shift}{\def\labelEdge@shift{#1}}
% ========= KEY DEFAULTS =========
\setkeys{labelEdge}{start=0,end=0,dist=1,xy=y,shift={0.3,0}}%
\newcommand{\labelEdge}[2][]{%label
	\begingroup
  \setkeys{labelEdge}{#1}% Set new keys
	\getxy{(\labelEdge@start)}{\xStart}{\yStart}
	\getxy{(\labelEdge@end)}{\xEnd}{\yEnd}
	\ifthenelse{\equal{\labelEdge@xy}{y}}
	{
		\coordinate (xshift) at (${(\xEnd-\xStart)/abs(\yEnd-\yStart)}*(\labelEdge@dist,0)$);
		\coordinate (yshift) at (${(\yEnd-\yStart)/abs(\yEnd-\yStart)}*((0,\labelEdge@dist)$);
	}{
		\coordinate (xshift) at (${(\xEnd-\xStart)/abs(\xEnd-\xStart)}*(\labelEdge@dist,0)$);
		\coordinate (yshift) at (${(\yEnd-\yStart)/abs(\xEnd-\xStart)}*((0,\labelEdge@dist)$);
	}
	\node (temp) at ($(\xStart,\yStart) + (xshift) + (yshift)$)	{};	
	\node[anchor=south] at ($(\labelEdge@shift)+(temp.south)$) {#2};
	\endgroup
}
% TOKEN
% ========= KEY DEFINITIONS =========
\define@key{token}{color}{\def\token@color{#1}}
% ========= KEY DEFAULTS =========
\setkeys{token}{color=white}%
\newcommand{\token}[2][]{%
	\begingroup
  \setkeys{token}{#1}% Set new keys
  \node[circle,minimum size=1.2mm,inner sep=0,draw,fill=\token@color] at (#2) {};
	\endgroup
}

% PORT
% ========= KEY DEFINITIONS =========
\define@key{port}{text}{\def\port@text{#1}}
\define@key{port}{color}{\def\port@color{#1}}
\define@key{port}{fill}{\def\port@fill{#1}}
\define@key{port}{id}{\def\port@id{#1}}
% ========= KEY DEFAULTS =========
\setkeys{port}{text={},color=black,fill=white,id=0}%
\newcommand{\port}[2][]{%
	\begingroup
  \setkeys{port}{#1}% Set new keys
  \node[circle,minimum size=5mm,inner sep=0.5mm,draw,\port@color,fill=\port@fill] (\port@id) at (#2) {\port@text};
	\endgroup
}

% NEGOTIATION
% ========= KEY DEFINITIONS =========
\define@key{nego}{text}{\def\nego@text{#1}}
%port count will be ignored if text is given
\define@key{nego}{ports}{\def\nego@ports{#1}}
\define@key{nego}{label}{\def\nego@label{#1}}
\define@key{nego}{color}{\def\nego@color{#1}}
\define@key{nego}{fill}{\def\nego@fill{#1}}
\define@key{nego}{id}{\def\nego@id{#1}}
\define@key{nego}{spacing}{\def\nego@spacing{#1}}
% ========= KEY DEFAULTS =========
\setkeys{nego}{text={},ports=0,label={},color=black,fill=white,id=0,spacing=1}%

\newcommand{\nego}[2][]{%argument: position
	\begingroup
	\setkeys{nego}{#1}
	\ifthenelse{\equal{\nego@text}{}}{
		%no text given
		\pgfmathsetmacro{\portcount}{\nego@ports-1}
		\foreach \x in {0,...,\portcount}
		{
			\port[color=\nego@color,fill=\nego@fill,id=\nego@id_P\x]{$(#2)+\nego@spacing*(\x,0)$};
		}
		\ifthenelse{\equal{\nego@ports}{1}}{
			\draw[line width=0.8mm] ($(#2)-(0.4,0)$) -- (\nego@id_P0) -- ($(#2)+(0.4,0)$);
		}{
			\foreach \x [remember=\x as \lastx (initially 0)] in {1,...,\portcount} {
				\draw[line width=0.8mm]  (\nego@id_P\lastx)-- (\nego@id_P\x);
			}
		}
	}{
		%text was given
		\StrLen{\nego@text}[\ports]
		\foreach \x [remember=\x as \lastx (initially 0)] in {1,...,\ports}
		{
			\port[text=\StrChar{\nego@text}{\x},color=\nego@color,fill=\nego@fill,id=\nego@id_P\lastx]{$(#2)+\nego@spacing*(\x-1,0)$};
		}
		
		\ifthenelse{\equal{\ports}{1}}{
			\draw[line width=0.8mm] ($(#2)-(0.4,0)$) -- (\nego@id_P0) -- ($(#2)+(0.4,0)$);
		}{
			\pgfmathsetmacro{\portcount}{\ports-1}
			\foreach \x [remember=\x as \lastx (initially 0)] in {1,...,\portcount} {
				\draw[line width=0.8mm]  (\nego@id_P\lastx)-- (\nego@id_P\x);
			}
		}
	}
	\endgroup%
}
\makeatother
